Improving Testsuites via Instrumentation

This paper explores the usefulness of a technique from software engineering, namely code instrumentation, for the development of large-scale natural language grammars. Information about the usage of grammar rules in test sentences is used to detect untested rules, redundant test sentences, and likely causes of overgeneration. Results show that less than half of a large-coverage grammar for German is actually tested by two large testsuites, and that 10-30% of testing time is redundant. The methodology applied can be seen as a re-use of grammar writing knowledge for testsuite compilation.

==> nobi-hyphen.tex <==
\hyphenation{
Adjektiv-endun-gen
Allo-morph-re-geln
Allo-morphe
Allo-morphie
Ana-lyse-pro-gramm
Analyse-protokoll
De-fini-tion
Dis-kurs-wissen
Hash-funk-tio-nen
Hash-funk-tion
Haupt-speicher
Im-ple-men-tation
Kate-gorien
Kla-ssi-fi-ka-tion
Kombi-nations-regeln
Lama
Lexikon-organi-sation
Nomina
Para-digma
Parti-zipI
%Pr"afixe
Pro-gramm
Sprach-ana-lyse-sys-tem
Sys-tems
TRUE
Teil-auf-gabe
Unifikations-formalis-mus
Verb-le-xi-kon
Verb-le-xi-kons
Wort-analysen
Wort-seman-tik
an-dere
aus-gehend
be-deutungs-tragende
be-nutzt
beruf-liche
buch-staben-orien-tiert
buch-staben-orien-tierten
dies
ka-te-go-ri-siert
morphem-orientiert
regexp
%re-pr"asentiert
spe-zielle
}

